Amazon SageMaker Model Monitor: A System for Real-Time Insights into Deployed Machine Learning Models

With the increasing adoption of machine learning (ML) models and systems in high-stakes settings across different industries, guaranteeing a model's performance after deployment has become crucial. Monitoring models in production is a critical aspect of ensuring their continued performance and reliability. We present Amazon SageMaker Model Monitor, a fully managed service that continuously monitors the quality of machine learning models hosted on Amazon SageMaker. Our system automatically detects data, concept, bias, and feature attribution drift in models in real-time and provides alerts so that model owners can take corrective actions and thereby maintain high quality models. We describe the key requirements obtained from customers, system design and architecture, and methodology for detecting different types of drift. Further, we provide quantitative evaluations followed by use cases, insights, and lessons learned from more than two years of production deployment.

==> figures/confusion.tex <==
 \begin{tikzpicture}[scale=0.5]
  \begin{axis}[
    view={0}{90},
    width=200,
    height=200,
    xmin=0,
    xmax=42,
    ymin=0,
    ymax=42,
    axis equal image,
    colormap/viridis
  ]
   \addplot3[matrix plot*] coordinates {
(0,0,33) (0,1,3) (0,2,0) (0,3,0) (0,4,1) (0,5,0) (0,6,0) (0,7,0) (0,8,3) (0,9,0) (0,10,0) (0,11,0) (0,12,0) (0,13,0) (0,14,0) (0,15,0) (0,16,0) (0,17,0) (0,18,0) (0,19,0) (0,20,0) (0,21,0) (0,22,0) (0,23,0) (0,24,0) (0,25,0) (0,26,0) (0,27,0) (0,28,0) (0,29,0) (0,30,0) (0,31,0) (0,32,0) (0,33,0) (0,34,0) (0,35,0) (0,36,0) (0,37,0) (0,38,0) (0,39,0) (0,40,0) (0,41,0) (0,42,0) 

(1,0,0) (1,1,40) (1,2,0) (1,3,0) (1,4,0) (1,5,0) (1,6,0) (1,7,0) (1,8,0) (1,9,0) (1,10,0) (1,11,0) (1,12,0) (1,13,0) (1,14,0) (1,15,0) (1,16,0) (1,17,0) (1,18,0) (1,19,0) (1,20,0) (1,21,0) (1,22,0) (1,23,0) (1,24,0) (1,25,0) (1,26,0) (1,27,0) (1,28,0) (1,29,0) (1,30,0) (1,31,0) (1,32,0) (1,33,0) (1,34,0) (1,35,0) (1,36,0) (1,37,0) (1,38,0) (1,39,0) (1,40,0) (1,41,0) (1,42,0) 

(2,0,0) (2,1,0) (2,2,40) (2,3,0) (2,4,0) (2,5,0) (2,6,0) (2,7,0) (2,8,0) (2,9,0) (2,10,0) (2,11,0) (2,12,0) (2,13,0) (2,14,0) (2,15,0) (2,16,0) (2,17,0) (2,18,0) (2,19,0) (2,20,0) (2,21,0) (2,22,0) (2,23,0) (2,24,0) (2,25,0) (2,26,0) (2,27,0) (2,28,0) (2,29,0) (2,30,0) (2,31,0) (2,32,0) (2,33,0) (2,34,0) (2,35,0) (2,36,0) (2,37,0) (2,38,0) (2,39,0) (2,40,0) (2,41,0) (2,42,0) 

(3,0,0) (3,1,0) (3,2,0) (3,3,39) (3,4,0) (3,5,1) (3,6,0) (3,7,0) (3,8,0) (3,9,0) (3,10,0) (3,11,0) (3,12,0) (3,13,0) (3,14,0) (3,15,0) (3,16,0) (3,17,0) (3,18,0) (3,19,0) (3,20,0) (3,21,0) (3,22,0) (3,23,0) (3,24,0) (3,25,0) (3,26,0) (3,27,0) (3,28,0) (3,29,0) (3,30,0) (3,31,0) (3,32,0) (3,33,0) (3,34,0) (3,35,0) (3,36,0) (3,37,0) (3,38,0) (3,39,0) (3,40,0) (3,41,0) (3,42,0) 

(4,0,0) (4,1,0) (4,2,0) (4,3,0) (4,4,39) (4,5,1) (4,6,0) (4,7,0) (4,8,0) (4,9,0) (4,10,0) (4,11,0) (4,12,0) (4,13,0) (4,14,0) (4,15,0) (4,16,0) (4,17,0) (4,18,0) (4,19,0) (4,20,0) (4,21,0) (4,22,0) (4,23,0) (4,24,0) (4,25,0) (4,26,0) (4,27,0) (4,28,0) (4,29,0) (4,30,0) (4,31,0) (4,32,0) (4,33,0) (4,34,0) (4,35,0) (4,36,0) (4,37,0) (4,38,0) (4,39,0) (4,40,0) (4,41,0) (4,42,0) 

(5,0,0) (5,1,0) (5,2,0) (5,3,0) (5,4,0) (5,5,40) (5,6,0) (5,7,0) (5,8,0) (5,9,0) (5,10,0) (5,11,0) (5,12,0) (5,13,0) (5,14,0) (5,15,0) (5,16,0) (5,17,0) (5,18,0) (5,19,0) (5,20,0) (5,21,0) (5,22,0) (5,23,0) (5,24,0) (5,25,0) (5,26,0) (5,27,0) (5,28,0) (5,29,0) (5,30,0) (5,31,0) (5,32,0) (5,33,0) (5,34,0) (5,35,0) (5,36,0) (5,37,0) (5,38,0) (5,39,0) (5,40,0) (5,41,0) (5,42,0) 

(6,0,0) (6,1,0) (6,2,0) (6,3,0) (6,4,0) (6,5,0) (6,6,40) (6,7,0) (6,8,0) (6,9,0) (6,10,0) (6,11,0) (6,12,0) (6,13,0) (6,14,0) (6,15,0) (6,16,0) (6,17,0) (6,18,0) (6,19,0) (6,20,0) (6,21,0) (6,22,0) (6,23,0) (6,24,0) (6,25,0) (6,26,0) (6,27,0) (6,28,0) (6,29,0) (6,30,0) (6,31,0) (6,32,0) (6,33,0) (6,34,0) (6,35,0) (6,36,0) (6,37,0) (6,38,0) (6,39,0) (6,40,0) (6,41,0) (6,42,0) 

(7,0,0) (7,1,0) (7,2,0) (7,3,0) (7,4,0) (7,5,0) (7,6,0) (7,7,40) (7,8,0) (7,9,0) (7,10,0) (7,11,0) (7,12,0) (7,13,0) (7,14,0) (7,15,0) (7,16,0) (7,17,0) (7,18,0) (7,19,0) (7,20,0) (7,21,0) (7,22,0) (7,23,0) (7,24,0) (7,25,0) (7,26,0) (7,27,0) (7,28,0) (7,29,0) (7,30,0) (7,31,0) (7,32,0) (7,33,0) (7,34,0) (7,35,0) (7,36,0) (7,37,0) (7,38,0) (7,39,0) (7,40,0) (7,41,0) (7,42,0) 

(8,0,0) (8,1,0) (8,2,0) (8,3,2) (8,4,0) (8,5,2) (8,6,0) (8,7,0) (8,8,36) (8,9,0) (8,10,0) (8,11,0) (8,12,0) (8,13,0) (8,14,0) (8,15,0) (8,16,0) (8,17,0) (8,18,0) (8,19,0) (8,20,0) (8,21,0) (8,22,0) (8,23,0) (8,24,0) (8,25,0) (8,26,0) (8,27,0) (8,28,0) (8,29,0) (8,30,0) (8,31,0) (8,32,0) (8,33,0) (8,34,0) (8,35,0) (8,36,0) (8,37,0) (8,38,0) (8,39,0) (8,40,0) (8,41,0) (8,42,0) 

(9,0,0) (9,1,0) (9,2,0) (9,3,0) (9,4,0) (9,5,0) (9,6,0) (9,7,0) (9,8,0) (9,9,40) (9,10,0) (9,11,0) (9,12,0) (9,13,0) (9,14,0) (9,15,0) (9,16,0) (9,17,0) (9,18,0) (9,19,0) (9,20,0) (9,21,0) (9,22,0) (9,23,0) (9,24,0) (9,25,0) (9,26,0) (9,27,0) (9,28,0) (9,29,0) (9,30,0) (9,31,0) (9,32,0) (9,33,0) (9,34,0) (9,35,0) (9,36,0) (9,37,0) (9,38,0) (9,39,0) (9,40,0) (9,41,0) (9,42,0) 

(10,0,0) (10,1,0) (10,2,0) (10,3,0) (10,4,0) (10,5,0) (10,6,0) (10,7,0) (10,8,0) (10,9,0) (10,10,40) (10,11,0) (10,12,0) (10,13,0) (10,14,0) (10,15,0) (10,16,0) (10,17,0) (10,18,0) (10,19,0) (10,20,0) (10,21,0) (10,22,0) (10,23,0) (10,24,0) (10,25,0) (10,26,0) (10,27,0) (10,28,0) (10,29,0) (10,30,0) (10,31,0) (10,32,0) (10,33,0) (10,34,0) (10,35,0) (10,36,0) (10,37,0) (10,38,0) (10,39,0) (10,40,0) (10,41,0) (10,42,0) 

(11,0,0) (11,1,0) (11,2,0) (11,3,0) (11,4,0) (11,5,0) (11,6,0) (11,7,0) (11,8,0) (11,9,0) (11,10,0) (11,11,40) (11,12,0) (11,13,0) (11,14,0) (11,15,0) (11,16,0) (11,17,0) (11,18,0) (11,19,0) (11,20,0) (11,21,0) (11,22,0) (11,23,0) (11,24,0) (11,25,0) (11,26,0) (11,27,0) (11,28,0) (11,29,0) (11,30,0) (11,31,0) (11,32,0) (11,33,0) (11,34,0) (11,35,0) (11,36,0) (11,37,0) (11,38,0) (11,39,0) (11,40,0) (11,41,0) (11,42,0) 

(12,0,0) (12,1,0) (12,2,0) (12,3,0) (12,4,0) (12,5,0) (12,6,0) (12,7,0) (12,8,0) (12,9,0) (12,10,0) (12,11,0) (12,12,40) (12,13,0) (12,14,0) (12,15,0) (12,16,0) (12,17,0) (12,18,0) (12,19,0) (12,20,0) (12,21,0) (12,22,0) (12,23,0) (12,24,0) (12,25,0) (12,26,0) (12,27,0) (12,28,0) (12,29,0) (12,30,0) (12,31,0) (12,32,0) (12,33,0) (12,34,0) (12,35,0) (12,36,0) (12,37,0) (12,38,0) (12,39,0) (12,40,0) (12,41,0) (12,42,0) 

(13,0,0) (13,1,0) (13,2,0) (13,3,0) (13,4,0) (13,5,0) (13,6,0) (13,7,0) (13,8,0) (13,9,0) (13,10,0) (13,11,0) (13,12,0) (13,13,40) (13,14,0) (13,15,0) (13,16,0) (13,17,0) (13,18,0) (13,19,0) (13,20,0) (13,21,0) (13,22,0) (13,23,0) (13,24,0) (13,25,0) (13,26,0) (13,27,0) (13,28,0) (13,29,0) (13,30,0) (13,31,0) (13,32,0) (13,33,0) (13,34,0) (13,35,0) (13,36,0) (13,37,0) (13,38,0) (13,39,0) (13,40,0) (13,41,0) (13,42,0) 

(14,0,0) (14,1,0) (14,2,0) (14,3,0) (14,4,0) (14,5,0) (14,6,0) (14,7,0) (14,8,0) (14,9,0) (14,10,0) (14,11,0) (14,12,0) (14,13,0) (14,14,40) (14,15,0) (14,16,0) (14,17,0) (14,18,0) (14,19,0) (14,20,0) (14,21,0) (14,22,0) (14,23,0) (14,24,0) (14,25,0) (14,26,0) (14,27,0) (14,28,0) (14,29,0) (14,30,0) (14,31,0) (14,32,0) (14,33,0) (14,34,0) (14,35,0) (14,36,0) (14,37,0) (14,38,0) (14,39,0) (14,40,0) (14,41,0) (14,42,0) 

(15,0,0) (15,1,0) (15,2,0) (15,3,0) (15,4,0) (15,5,0) (15,6,0) (15,7,0) (15,8,0) (15,9,0) (15,10,0) (15,11,0) (15,12,0) (15,13,0) (15,14,0) (15,15,40) (15,16,0) (15,17,0) (15,18,0) (15,19,0) (15,20,0) (15,21,0) (15,22,0) (15,23,0) (15,24,0) (15,25,0) (15,26,0) (15,27,0) (15,28,0) (15,29,0) (15,30,0) (15,31,0) (15,32,0) (15,33,0) (15,34,0) (15,35,0) (15,36,0) (15,37,0) (15,38,0) (15,39,0) (15,40,0) (15,41,0) (15,42,0) 

(16,0,0) (16,1,0) (16,2,0) (16,3,1) (16,4,0) (16,5,0) (16,6,0) (16,7,0) (16,8,0) (16,9,0) (16,10,0) (16,11,0) (16,12,0) (16,13,0) (16,14,0) (16,15,0) (16,16,39) (16,17,0) (16,18,0) (16,19,0) (16,20,0) (16,21,0) (16,22,0) (16,23,0) (16,24,0) (16,25,0) (16,26,0) (16,27,0) (16,28,0) (16,29,0) (16,30,0) (16,31,0) (16,32,0) (16,33,0) (16,34,0) (16,35,0) (16,36,0) (16,37,0) (16,38,0) (16,39,0) (16,40,0) (16,41,0) (16,42,0) 

(17,0,0) (17,1,0) (17,2,0) (17,3,0) (17,4,0) (17,5,0) (17,6,0) (17,7,0) (17,8,0) (17,9,0) (17,10,0) (17,11,0) (17,12,0) (17,13,0) (17,14,0) (17,15,0) (17,16,0) (17,17,40) (17,18,0) (17,19,0) (17,20,0) (17,21,0) (17,22,0) (17,23,0) (17,24,0) (17,25,0) (17,26,0) (17,27,0) (17,28,0) (17,29,0) (17,30,0) (17,31,0) (17,32,0) (17,33,0) (17,34,0) (17,35,0) (17,36,0) (17,37,0) (17,38,0) (17,39,0) (17,40,0) (17,41,0) (17,42,0) 

(18,0,0) (18,1,0) (18,2,0) (18,3,0) (18,4,0) (18,5,0) (18,6,0) (18,7,0) (18,8,0) (18,9,0) (18,10,0) (18,11,0) (18,12,0) (18,13,0) (18,14,0) (18,15,0) (18,16,0) (18,17,0) (18,18,40) (18,19,0) (18,20,0) (18,21,0) (18,22,0) (18,23,0) (18,24,0) (18,25,0) (18,26,0) (18,27,0) (18,28,0) (18,29,0) (18,30,0) (18,31,0) (18,32,0) (18,33,0) (18,34,0) (18,35,0) (18,36,0) (18,37,0) (18,38,0) (18,39,0) (18,40,0) (18,41,0) (18,42,0) 

(19,0,0) (19,1,0) (19,2,0) (19,3,0) (19,4,0) (19,5,0) (19,6,0) (19,7,0) (19,8,0) (19,9,0) (19,10,0) (19,11,1) (19,12,0) (19,13,0) (19,14,0) (19,15,0) (19,16,0) (19,17,0) (19,18,0) (19,19,24) (19,20,12) (19,21,3) (19,22,0) (19,23,0) (19,24,0) (19,25,0) (19,26,0) (19,27,0) (19,28,0) (19,29,0) (19,30,0) (19,31,0) (19,32,0) (19,33,0) (19,34,0) (19,35,0) (19,36,0) (19,37,0) (19,38,0) (19,39,0) (19,40,0) (19,41,0) (19,42,0) 

(20,0,0) (20,1,0) (20,2,0) (20,3,0) (20,4,0) (20,5,0) (20,6,0) (20,7,0) (20,8,0) (20,9,0) (20,10,0) (20,11,0) (20,12,0) (20,13,0) (20,14,0) (20,15,0) (20,16,0) (20,17,0) (20,18,0) (20,19,21) (20,20,15) (20,21,3) (20,22,0) (20,23,0) (20,24,0) (20,25,1) (20,26,0) (20,27,0) (20,28,0) (20,29,0) (20,30,0) (20,31,0) (20,32,0) (20,33,0) (20,34,0) (20,35,0) (20,36,0) (20,37,0) (20,38,0) (20,39,0) (20,40,0) (20,41,0) (20,42,0) 

(21,0,0) (21,1,0) (21,2,0) (21,3,0) (21,4,0) (21,5,0) (21,6,0) (21,7,0) (21,8,0) (21,9,0) (21,10,0) (21,11,2) (21,12,0) (21,13,0) (21,14,0) (21,15,0) (21,16,0) (21,17,0) (21,18,0) (21,19,0) (21,20,0) (21,21,38) (21,22,0) (21,23,0) (21,24,0) (21,25,0) (21,26,0) (21,27,0) (21,28,0) (21,29,0) (21,30,0) (21,31,0) (21,32,0) (21,33,0) (21,34,0) (21,35,0) (21,36,0) (21,37,0) (21,38,0) (21,39,0) (21,40,0) (21,41,0) (21,42,0) 

(22,0,0) (22,1,0) (22,2,0) (22,3,0) (22,4,0) (22,5,0) (22,6,0) (22,7,0) (22,8,0) (22,9,0) (22,10,0) (22,11,0) (22,12,0) (22,13,0) (22,14,0) (22,15,0) (22,16,0) (22,17,0) (22,18,0) (22,19,0) (22,20,0) (22,21,0) (22,22,30) (22,23,0) (22,24,0) (22,25,10) (22,26,0) (22,27,0) (22,28,0) (22,29,0) (22,30,0) (22,31,0) (22,32,0) (22,33,0) (22,34,0) (22,35,0) (22,36,0) (22,37,0) (22,38,0) (22,39,0) (22,40,0) (22,41,0) (22,42,0) 

(23,0,0) (23,1,0) (23,2,0) (23,3,0) (23,4,0) (23,5,0) (23,6,0) (23,7,0) (23,8,0) (23,9,0) (23,10,0) (23,11,0) (23,12,0) (23,13,0) (23,14,0) (23,15,0) (23,16,0) (23,17,0) (23,18,0) (23,19,0) (23,20,0) (23,21,0) (23,22,0) (23,23,38) (23,24,0) (23,25,0) (23,26,0) (23,27,0) (23,28,0) (23,29,0) (23,30,0) (23,31,2) (23,32,0) (23,33,0) (23,34,0) (23,35,0) (23,36,0) (23,37,0) (23,38,0) (23,39,0) (23,40,0) (23,41,0) (23,42,0) 

(24,0,0) (24,1,0) (24,2,0) (24,3,0) (24,4,0) (24,5,0) (24,6,0) (24,7,0) (24,8,0) (24,9,0) (24,10,0) (24,11,0) (24,12,0) (24,13,0) (24,14,0) (24,15,0) (24,16,0) (24,17,0) (24,18,0) (24,19,0) (24,20,0) (24,21,0) (24,22,0) (24,23,0) (24,24,39) (24,25,1) (24,26,0) (24,27,0) (24,28,0) (24,29,0) (24,30,0) (24,31,0) (24,32,0) (24,33,0) (24,34,0) (24,35,0) (24,36,0) (24,37,0) (24,38,0) (24,39,0) (24,40,0) (24,41,0) (24,42,0) 

(25,0,0) (25,1,0) (25,2,0) (25,3,0) (25,4,0) (25,5,0) (25,6,0) (25,7,0) (25,8,0) (25,9,0) (25,10,0) (25,11,0) (25,12,0) (25,13,0) (25,14,0) (25,15,0) (25,16,0) (25,17,0) (25,18,0) (25,19,0) (25,20,0) (25,21,0) (25,22,0) (25,23,0) (25,24,0) (25,25,40) (25,26,0) (25,27,0) (25,28,0) (25,29,0) (25,30,0) (25,31,0) (25,32,0) (25,33,0) (25,34,0) (25,35,0) (25,36,0) (25,37,0) (25,38,0) (25,39,0) (25,40,0) (25,41,0) (25,42,0) 

(26,0,0) (26,1,0) (26,2,0) (26,3,0) (26,4,0) (26,5,0) (26,6,0) (26,7,0) (26,8,0) (26,9,0) (26,10,0) (26,11,0) (26,12,0) (26,13,0) (26,14,0) (26,15,0) (26,16,0) (26,17,0) (26,18,1) (26,19,0) (26,20,0) (26,21,0) (26,22,0) (26,23,0) (26,24,0) (26,25,0) (26,26,39) (26,27,0) (26,28,0) (26,29,0) (26,30,0) (26,31,0) (26,32,0) (26,33,0) (26,34,0) (26,35,0) (26,36,0) (26,37,0) (26,38,0) (26,39,0) (26,40,0) (26,41,0) (26,42,0) 

(27,0,0) (27,1,0) (27,2,0) (27,3,0) (27,4,0) (27,5,0) (27,6,0) (27,7,0) (27,8,0) (27,9,0) (27,10,0) (27,11,0) (27,12,0) (27,13,0) (27,14,0) (27,15,0) (27,16,0) (27,17,0) (27,18,0) (27,19,0) (27,20,0) (27,21,0) (27,22,0) (27,23,0) (27,24,0) (27,25,16) (27,26,0) (27,27,24) (27,28,0) (27,29,0) (27,30,0) (27,31,0) (27,32,0) (27,33,0) (27,34,0) (27,35,0) (27,36,0) (27,37,0) (27,38,0) (27,39,0) (27,40,0) (27,41,0) (27,42,0) 

(28,0,0) (28,1,0) (28,2,0) (28,3,0) (28,4,0) (28,5,0) (28,6,0) (28,7,0) (28,8,0) (28,9,0) (28,10,0) (28,11,0) (28,12,0) (28,13,0) (28,14,0) (28,15,0) (28,16,0) (28,17,0) (28,18,0) (28,19,0) (28,20,0) (28,21,0) (28,22,0) (28,23,0) (28,24,0) (28,25,0) (28,26,0) (28,27,0) (28,28,40) (28,29,0) (28,30,0) (28,31,0) (28,32,0) (28,33,0) (28,34,0) (28,35,0) (28,36,0) (28,37,0) (28,38,0) (28,39,0) (28,40,0) (28,41,0) (28,42,0) 

(29,0,0) (29,1,0) (29,2,0) (29,3,0) (29,4,0) (29,5,0) (29,6,0) (29,7,0) (29,8,0) (29,9,0) (29,10,0) (29,11,0) (29,12,0) (29,13,0) (29,14,0) (29,15,0) (29,16,0) (29,17,0) (29,18,0) (29,19,0) (29,20,0) (29,21,0) (29,22,1) (29,23,0) (29,24,0) (29,25,1) (29,26,0) (29,27,0) (29,28,1) (29,29,36) (29,30,1) (29,31,0) (29,32,0) (29,33,0) (29,34,0) (29,35,0) (29,36,0) (29,37,0) (29,38,0) (29,39,0) (29,40,0) (29,41,0) (29,42,0) 

(30,0,0) (30,1,0) (30,2,0) (30,3,0) (30,4,0) (30,5,0) (30,6,0) (30,7,0) (30,8,0) (30,9,0) (30,10,0) (30,11,6) (30,12,0) (30,13,0) (30,14,0) (30,15,0) (30,16,0) (30,17,0) (30,18,0) (30,19,0) (30,20,0) (30,21,0) (30,22,0) (30,23,0) (30,24,0) (30,25,1) (30,26,0) (30,27,0) (30,28,0) (30,29,0) (30,30,33) (30,31,0) (30,32,0) (30,33,0) (30,34,0) (30,35,0) (30,36,0) (30,37,0) (30,38,0) (30,39,0) (30,40,0) (30,41,0) (30,42,0) 

(31,0,0) (31,1,0) (31,2,0) (31,3,0) (31,4,0) (31,5,0) (31,6,0) (31,7,0) (31,8,0) (31,9,0) (31,10,0) (31,11,0) (31,12,0) (31,13,0) (31,14,0) (31,15,0) (31,16,0) (31,17,0) (31,18,0) (31,19,0) (31,20,0) (31,21,0) (31,22,0) (31,23,0) (31,24,0) (31,25,0) (31,26,0) (31,27,0) (31,28,0) (31,29,0) (31,30,0) (31,31,40) (31,32,0) (31,33,0) (31,34,0) (31,35,0) (31,36,0) (31,37,0) (31,38,0) (31,39,0) (31,40,0) (31,41,0) (31,42,0) 

(32,0,0) (32,1,0) (32,2,0) (32,3,0) (32,4,0) (32,5,0) (32,6,0) (32,7,0) (32,8,0) (32,9,0) (32,10,0) (32,11,0) (32,12,0) (32,13,0) (32,14,0) (32,15,0) (32,16,0) (32,17,0) (32,18,0) (32,19,0) (32,20,0) (32,21,0) (32,22,0) (32,23,0) (32,24,0) (32,25,0) (32,26,0) (32,27,0) (32,28,0) (32,29,0) (32,30,0) (32,31,0) (32,32,40) (32,33,0) (32,34,0) (32,35,0) (32,36,0) (32,37,0) (32,38,0) (32,39,0) (32,40,0) (32,41,0) (32,42,0) 

(33,0,0) (33,1,0) (33,2,0) (33,3,0) (33,4,0) (33,5,0) (33,6,0) (33,7,0) (33,8,0) (33,9,0) (33,10,0) (33,11,0) (33,12,0) (33,13,0) (33,14,0) (33,15,0) (33,16,0) (33,17,0) (33,18,0) (33,19,0) (33,20,0) (33,21,0) (33,22,0) (33,23,0) (33,24,0) (33,25,0) (33,26,0) (33,27,0) (33,28,0) (33,29,0) (33,30,0) (33,31,0) (33,32,0) (33,33,40) (33,34,0) (33,35,0) (33,36,0) (33,37,0) (33,38,0) (33,39,0) (33,40,0) (33,41,0) (33,42,0) 

(34,0,0) (34,1,0) (34,2,0) (34,3,0) (34,4,0) (34,5,0) (34,6,0) (34,7,0) (34,8,0) (34,9,0) (34,10,0) (34,11,0) (34,12,0) (34,13,0) (34,14,0) (34,15,0) (34,16,0) (34,17,0) (34,18,0) (34,19,0) (34,20,0) (34,21,0) (34,22,0) (34,23,0) (34,24,0) (34,25,0) (34,26,0) (34,27,0) (34,28,0) (34,29,0) (34,30,0) (34,31,0) (34,32,0) (34,33,0) (34,34,40) (34,35,0) (34,36,0) (34,37,0) (34,38,0) (34,39,0) (34,40,0) (34,41,0) (34,42,0) 

(35,0,0) (35,1,0) (35,2,0) (35,3,0) (35,4,0) (35,5,0) (35,6,0) (35,7,0) (35,8,0) (35,9,0) (35,10,0) (35,11,0) (35,12,0) (35,13,0) (35,14,0) (35,15,0) (35,16,0) (35,17,0) (35,18,0) (35,19,0) (35,20,0) (35,21,0) (35,22,0) (35,23,0) (35,24,0) (35,25,0) (35,26,0) (35,27,0) (35,28,0) (35,29,0) (35,30,0) (35,31,0) (35,32,0) (35,33,0) (35,34,0) (35,35,40) (35,36,0) (35,37,0) (35,38,0) (35,39,0) (35,40,0) (35,41,0) (35,42,0) 

(36,0,0) (36,1,0) (36,2,0) (36,3,0) (36,4,0) (36,5,0) (36,6,0) (36,7,0) (36,8,0) (36,9,0) (36,10,0) (36,11,0) (36,12,0) (36,13,0) (36,14,0) (36,15,0) (36,16,0) (36,17,0) (36,18,0) (36,19,0) (36,20,0) (36,21,0) (36,22,0) (36,23,0) (36,24,0) (36,25,0) (36,26,0) (36,27,0) (36,28,0) (36,29,0) (36,30,0) (36,31,0) (36,32,0) (36,33,0) (36,34,0) (36,35,0) (36,36,40) (36,37,0) (36,38,0) (36,39,0) (36,40,0) (36,41,0) (36,42,0) 

(37,0,0) (37,1,0) (37,2,0) (37,3,0) (37,4,0) (37,5,0) (37,6,0) (37,7,0) (37,8,0) (37,9,0) (37,10,0) (37,11,0) (37,12,0) (37,13,0) (37,14,0) (37,15,0) (37,16,0) (37,17,0) (37,18,0) (37,19,0) (37,20,0) (37,21,0) (37,22,0) (37,23,0) (37,24,0) (37,25,0) (37,26,0) (37,27,0) (37,28,0) (37,29,0) (37,30,0) (37,31,0) (37,32,0) (37,33,1) (37,34,0) (37,35,0) (37,36,35) (37,37,4) (37,38,0) (37,39,0) (37,40,0) (37,41,0) (37,42,0) 

(38,0,0) (38,1,0) (38,2,0) (38,3,0) (38,4,0) (38,5,0) (38,6,0) (38,7,0) (38,8,0) (38,9,0) (38,10,0) (38,11,0) (38,12,0) (38,13,0) (38,14,0) (38,15,0) (38,16,0) (38,17,0) (38,18,0) (38,19,0) (38,20,0) (38,21,0) (38,22,0) (38,23,0) (38,24,0) (38,25,0) (38,26,0) (38,27,0) (38,28,0) (38,29,0) (38,30,0) (38,31,0) (38,32,0) (38,33,0) (38,34,0) (38,35,0) (38,36,0) (38,37,0) (38,38,40) (38,39,0) (38,40,0) (38,41,0) (38,42,0) 

(39,0,0) (39,1,0) (39,2,0) (39,3,0) (39,4,0) (39,5,0) (39,6,0) (39,7,0) (39,8,0) (39,9,0) (39,10,0) (39,11,0) (39,12,0) (39,13,0) (39,14,0) (39,15,0) (39,16,0) (39,17,0) (39,18,0) (39,19,0) (39,20,0) (39,21,0) (39,22,0) (39,23,0) (39,24,0) (39,25,0) (39,26,0) (39,27,0) (39,28,0) (39,29,0) (39,30,0) (39,31,0) (39,32,0) (39,33,0) (39,34,0) (39,35,0) (39,36,0) (39,37,0) (39,38,35) (39,39,5) (39,40,0) (39,41,0) (39,42,0) 

(40,0,0) (40,1,0) (40,2,0) (40,3,0) (40,4,0) (40,5,0) (40,6,0) (40,7,0) (40,8,0) (40,9,0) (40,10,0) (40,11,0) (40,12,0) (40,13,0) (40,14,0) (40,15,0) (40,16,0) (40,17,0) (40,18,0) (40,19,0) (40,20,0) (40,21,0) (40,22,0) (40,23,0) (40,24,0) (40,25,0) (40,26,0) (40,27,0) (40,28,0) (40,29,0) (40,30,0) (40,31,0) (40,32,0) (40,33,2) (40,34,1) (40,35,0) (40,36,0) (40,37,0) (40,38,0) (40,39,0) (40,40,37) (40,41,0) (40,42,0) 

(41,0,0) (41,1,0) (41,2,0) (41,3,0) (41,4,0) (41,5,0) (41,6,1) (41,7,0) (41,8,0) (41,9,3) (41,10,0) (41,11,0) (41,12,0) (41,13,0) (41,14,0) (41,15,0) (41,16,0) (41,17,0) (41,18,0) (41,19,0) (41,20,0) (41,21,0) (41,22,0) (41,23,0) (41,24,0) (41,25,0) (41,26,0) (41,27,0) (41,28,0) (41,29,0) (41,30,0) (41,31,0) (41,32,0) (41,33,0) (41,34,0) (41,35,0) (41,36,0) (41,37,0) (41,38,0) (41,39,0) (41,40,0) (41,41,36) (41,42,0) 

(42,0,0) (42,1,1) (42,2,2) (42,3,0) (42,4,6) (42,5,0) (42,6,3) (42,7,0) (42,8,0) (42,9,0) (42,10,0) (42,11,0) (42,12,0) (42,13,0) (42,14,0) (42,15,0) (42,16,0) (42,17,0) (42,18,0) (42,19,0) (42,20,1) (42,21,0) (42,22,0) (42,23,0) (42,24,0) (42,25,0) (42,26,0) (42,27,0) (42,28,0) (42,29,0) (42,30,0) (42,31,0) (42,32,0) (42,33,0) (42,34,0) (42,35,0) (42,36,0) (42,37,0) (42,38,0) (42,39,0) (42,40,0) (42,41,6) (42,42,21)};
  \end{axis}
 \end{tikzpicture}

==> figures/mlpipeline.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,478); %set diagram left start at 0, and has height of 478

%Shape: Rectangle [id:dp8304228673417838] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (35,68) -- (180.5,68) -- (180.5,118) -- (35,118) -- cycle ;
%Shape: Rectangle [id:dp0063809559848235775] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (35,160) -- (189,160) -- (189,210) -- (35,210) -- cycle ;
%Shape: Rectangle [id:dp9526530501050406] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (36,282) -- (187,282) -- (187,332) -- (36,332) -- cycle ;
%Shape: Rectangle [id:dp5056882594388904] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (44,380) -- (183,380) -- (183,430) -- (44,430) -- cycle ;
%Straight Lines [id:da44417812562650516] 
\draw    (111,118.5) -- (111,158.5) ;
\draw [shift={(111,160.5)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da022778553822190184] 
\draw    (110.7,208.95) -- (110.7,275.95) ;
\draw [shift={(110.7,277.95)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6915412790813892] 
\draw    (112,334.5) -- (112,377.5) ;
\draw [shift={(112,379.5)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Arc [id:dp15132440568704064] 
\draw  [draw opacity=0] (110.7,208.95) .. controls (100.42,226.99) and (78.25,238.42) .. (53.71,236.26) .. controls (21.47,233.43) and (-2.65,208.23) .. (-0.17,179.98) .. controls (2.31,151.73) and (30.46,131.12) .. (62.69,133.95) .. controls (82.05,135.65) and (98.48,145.42) .. (107.99,159.07) -- (58.2,185.11) -- cycle ; \draw   (110.7,208.95) .. controls (100.42,226.99) and (78.25,238.42) .. (53.71,236.26) .. controls (21.47,233.43) and (-2.65,208.23) .. (-0.17,179.98) .. controls (2.31,151.73) and (30.46,131.12) .. (62.69,133.95) .. controls (82.05,135.65) and (98.48,145.42) .. (107.99,159.07) ;

% Text Node
\draw (50,85) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large 1. Prepare data }};
% Text Node
\draw (44,174) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large 2. Train and tune}\\{\large  \ \ \ \ \ \ \ \ \ \ \ model}};
% Text Node
\draw (50,290) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large 3. Deploy model}};
% Text Node
\draw (67,393) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large 4. Deployment}};
% Text Node
\draw (199,75) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large \textbf{Feature engineering}}\\{\large \textbf{Detect data issues }}};
% Text Node
\draw (199,160) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large \textbf{Detect training issues}}\\ {\large \textbf{Auto-terminate training jobs}}\\ \textbf{{\large Get model insights}}};

\draw (199,290) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large \textbf{Detect issues in tuning jobs}}\\ {\large \textbf{Auto-terminate tuning jobs}}};

% Text Node
\draw (199,394) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large \textbf{Understand predictions}}};


\end{tikzpicture}


==> figures/model_pruning.tex <==
x          y        meta
11181642    0.874   11.1M
9879482    0.8896   9.8M
8577898    0.8956   9.5M
7244058    0.8999   7.2M
6031754    0.8977   6.0M
4894906    0.8918   4.8M
3721770    0.8833   3.7M
2586074    0.8783   2.5M

==> figures/model_pruning2.tex <==
x          y    meta
1166210 0.8306  1.1M
267250  0.603   260k

==> figures/workflow.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,482); %set diagram left start at 0, and has height of 482

%Shape: Rectangle [id:dp4414106502315095] 
\draw   (25,22) -- (441.5,22) -- (441.5,95.8) -- (25,95.8) -- cycle ;
%Shape: Rectangle [id:dp571056943534144] 
%\draw   (84.88,151.28) -- (240.62,151.28) -- (240.62,196.08) -- (84.88,196.08) -- cycle ;
%Shape: Rectangle [id:dp5162019435310953] 
\draw   (39,282) -- (268.5,282) -- (268.5,352.8) -- (39,352.8) -- cycle ;
%Shape: Rectangle [id:dp8755085624494887] 
%\draw   (117.5,393) -- (383.5,393) -- (383.5,464.8) -- (117.5,464.8) -- cycle ;
%Straight Lines [id:da09856840457747529] 
\draw    (159.5,97.8) -- (159.5,147.8) ;
\draw [shift={(159.5,149.8)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da44011514881023917] 
\draw    (157.5,350.8) -- (190.5,388.8) ;
\draw [shift={(191.5,390.8)}, rotate = 232] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da39096990910189755] 
\draw    (158.5,280.8) -> (158.5,215.8) ;
\draw [shift={(158.5,215.8)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp6789043762758553] 
%\draw   (303,257.8) -- (417.5,257.8) -- (417.5,324.8) -- (303,324.8) -- cycle ;
%Straight Lines [id:da4627844635627337] 
\draw    (300.5,393) -- (355.5,329.8) ;
\draw [shift={(355.5,327.8)}, rotate = 120] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6608308676780037] 
\draw    (351.5,255.8) -- (350.51,98.8) ;
\draw [shift={(350.5,96.8)}, rotate = 449.64] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (90,30) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{{\LARGE SageMaker Training Container}}};
% Text Node
\draw (170,59) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large smdebug hook}};
% Text Node
\draw (60.25,168) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{{S3 Bucket}}};
\draw (125.25,148) node [anchor=north west][inner sep=0.75pt]   [align=left] {\includegraphics[scale=1]{figures/S3.png}};
% Text Node
\draw (68,107) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large S3Agent}};
% Text Node
\draw (80.25,285) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{{\LARGE Rule Container}}};
% Text Node
\draw (100.25,320) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large smdebug rule}};
% Text Node
\draw (200,470) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textbf{Cloudwatch Alarm}};
\draw (200,380) node [anchor=north west][inner sep=0.75pt]   [align=left] {\includegraphics[scale=1.3]{figures/cloudwatch.png}};
% Text Node
\draw (30,245) node [anchor=north west][inner sep=0.75pt]  [align=left] {{\Large smdebug trial}};
% Text Node
\draw (400,280.2) node [anchor=north west][inner sep=0.75pt]   [align=left] { \textbf{Lambda} \\ \textbf{Function}};
\draw (315,250.2) node [anchor=north west][inner sep=0.75pt]   [align=left] {\includegraphics[scale=1.2]{figures/lambda.png}};
% Text Node
\draw (362,166) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\Large Stop}\\{\Large Training}};


\end{tikzpicture}

